Single-Image Super-Resolution Reconstruction based on the Differences of Neighboring Pixels

The deep learning technique was used to increase the performance of single image super-resolution (SISR). However, most existing CNN-based SISR approaches primarily focus on establishing deeper or larger networks to extract more significant high-level features. Usually, the pixel-level loss between the target high-resolution image and the estimated image is used, but the neighbor relations between pixels in the image are seldom used. On the other hand, according to observations, a pixel's neighbor relationship contains rich information about the spatial structure, local context, and structural knowledge. Based on this fact, in this paper, we utilize pixel's neighbor relationships in a different perspective, and we propose the differences of neighboring pixels to regularize the CNN by constructing a graph from the estimated image and the ground-truth image. The proposed method outperforms the state-of-the-art methods in terms of quantitative and qualitative evaluation of the benchmark datasets. Keywords: Super-resolution, Convolutional Neural Networks, Deep Learning

==> tmp.tex <==
\textcolor{red}{We conduct anime-likes images Super-Resolution experiments on three datasets: Urban100\cite{huang2015}, BSD100\cite{martin2001} and Manga109\cite{manga109}. Cartoon Set is a collection of random, 2D cartoon avatar images. The cartoons vary in 10 artwork categories, 4 color categories, and 4 proportion categories, with a total of ~1013 possible combinations. We started our experiment on this simple dataset at first. 
Manga109 has been compiled by the Aizawa Yamasaki Matsui Laboratory, Department of Information and Communication Engineering, the Graduate School of Information Science and Technology, the University of Tokyo. The compilation is intended for use in academic research on the media processing of Japanese manga. 
We resized all samples to 128x128 pixels. We took 1k images for training and 100 images for testing.}

\textcolor{red}{We adopt the SRCNN\cite{dong2014} model as our baseline model due to its great performance on image super-resolution tasks. In all these settings, we compare the performance with and without our regularizer. We set 4000 epochs and batch size to 20. The learning rate is initialized to 0.0001 and halved at every 2000 epochs. We used Momentum as the optimization of the network. The proposed approach is implemented using Tensorflow library with Intel(R) Core(TM) i7-6700K CPU @ 4.00GHz Processor, 32 GB of RAM, and Nvidia GeForce RTX 3090 graphic cards.}
